StEP: Style-based Encoder Pre-training for Multi-modal Image Synthesis

We propose a novel approach for multi-modal Image-to-image (I2I) translation. To tackle the one-to-many relationship between input and output domains, previous works use complex training objectives to learn a latent embedding, jointly with the generator, that models the variability of the output domain. In contrast, we directly model the style variability of images, independent of the image synthesis task. Specifically, we pre-train a generic style encoder using a novel proxy task to learn an embedding of images, from arbitrary domains, into a low-dimensional style latent space. The learned latent space introduces several advantages over previous traditional approaches to multi-modal I2I translation. First, it is not dependent on the target dataset, and generalizes well across multiple domains. Second, it learns a more powerful and expressive latent space, which improves the fidelity of style capture and transfer. The proposed style pre-training also simplifies the training objective and speeds up the training significantly. Furthermore, we provide a detailed study of the contribution of different loss terms to the task of multi-modal I2I translation, and propose a simple alternative to VAEs to enable sampling from unconstrained latent spaces. Finally, we achieve state-of-the-art results on six challenging benchmarks with a simple training objective that includes only a GAN loss and a reconstruction loss.

==> figures_tex/user_study.tex <==
\begin{figure*}[ht!]
    \centering
    \captionsetup[subfigure]{aboveskip=1pt,belowskip=3pt}
    \begin{subfigure}[b]{0.6\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/user_study/user_study2.pdf}\\
        % \caption{Example question 1: which looks the more realistic, which is the main factor}
        \caption{Example question 1: realism is the main factor for choosing a preference.}
    \end{subfigure}
    \begin{subfigure}[b]{0.6\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/user_study/user_study.pdf}\\
        \caption{Example question 2: if both outputs have the same level of realism, then the user chooses the output that better matches the style image.}
    \end{subfigure}

    % \caption{Each question shows a sketch of a shoe and below it a real shoe from which we want to capture the style (color and texture) and transfer it to the sketch. Bottom left and bottom right are the outputs of two different methods. Choose which method (Left vs Right) generates a more \textbf{realistic} output with similar style to that of the style image (middle). You should compare the two methods based on (a) which looks the more realistic, which is the main factor, and (b) if both have the same level of realism, then which one better matches the style image.}
    \caption{Instructions and sample questions given in our user study. Each question shows a sketch of a shoe and below it a real shoe from which we want to capture the style (color and texture) and transfer it to the sketch. Bottom left and bottom right are the outputs of two different methods. The user chooses which method (left vs right) generates a more realistic output with similar style to that of the style image (middle). The user compares the two methods based on (a) which looks the more realistic, and (b) if both have the same level of realism, then which one better matches the style image.}
    \label{fig:user_study}
\end{figure*}

==> other_files/approach_old.tex <==
\section{Approach}
\subsection{Appearance modeling}
\label{sec:appearance_modeling}
To capture the one-to-many relationship between input viewpoints (represented by their deep buffers $B_i$) and output images $I_i$ under different appearances, we cast the rerendering task as a multimodal image translation~\cite{zhu2017toward}. 
In such a formulation, the goal is to learn a latent appearance vector $\za_i$ that captures variations in the output domain $I_i$ that cannot be inferred from the input domain $B_i$.
We compute the latent appearance vector as $\za_i = E^a(I_i, B_i)$ where $E^a$ is an appearance encoder that takes as input both the output image $I_i$ and the deep buffer $B_i$. 
We argue that having the appearance encoder $E^a$ observe the input $B_i$ allows it to  learn more complex appearance models by correlating the lighting in $I_i$ with scene geometry in $B_i$.
Finally, a rerendering network $R$ generates a scene rendering conditioned on both viewpoint $B_i$ and the latent appearance vector $\za$.

To train the appearance encoder $E^a$ and the rendering network $R$, we first adopted elements from state-of-the-art methods in multimodal synthesis~\cite{huang2018multimodal,lee2018diverse,zhu2017toward} to obtain a combination that is most effective in our scenario. 
However, this combination still has shortcomings as it is not able to model less-common appearances well.
For instance, it does not reliably capture night appearances for different scenes in our datasets.
We hypothesize that the appearance encoder (which is jointly trained with the rendering network) is not expressive enough to capture the large variability in the data.

In order to improve its expressiveness, we consider stabilizing the joint training of $R$ and $E^a$ by pretraining the appearance network $E^a$ independently on a proxy task.
We then employ a staged training approach in which the rendering network $R$ is first trained using fixed appearance embeddings, and finally we fine-tune both networks. 
This staged training regime allows for a simpler model that captures more complex appearances.

Next we present our baseline approach, which adapts state-of-the-art multimodal synthesis techniques, and our staged training strategy which pretrains the appearance encoder on a proxy task.

% final 
% Although the pretrained appearance embeddings do not match the appearance 
% Not only we observed improvements with the pretraining approach, but we also realized that 

% combined them in  maximize the reconstruction loss.
% However, that
% To tr

% While in~\cite{zhu2017unpaired} the appearance is captured from the ground truth output image $I_i$, we augment it with the corresponding deep buffer $B_i$.
% This can help the appearance encoder $E^a$ learn a more complex appearance model; for instance, it can correlate lighting in $I_i$ with scene geometry from $B_i$.

% We define the  latent appearance vector as $\za_i = E^a(I_i, B_i)$,. The rerendering network $R$ learns a joint mapping from input viewpoint and latent appearance to the real images, $R(B_i, \za_i) \rightarrow I_i$.
% % By changing $\za_i$, we can achieve multimodal rerendering for a single viewpoint.
% % Also by fixing it, we can have a consistent appearance with respect to viewpoint changes.
% To learn the latent appearance embedding, we explore two approaches: a baseline approach based on BicycleGAN~\cite{hiep2009towards}, and a new staged training method, where we first pretrain the appearance encoder $E^a$, then use the learned appearance embedding to train the rerendering network $R(B_i, \za_i)$.
% ------------------------------------------------------------------------------------------------

\paragraph{Baseline}
Our baseline is based on BicycleGAN~\cite{zhu2017toward} with two main differences.
First, our appearance encoder also takes as input the buffer~$B_i$, as described above.
Second, we add a cross-cycle consistency loss similar to~\cite{huang2018multimodal,lee2018diverse} to encourage appearance transfer across viewpoints.
Let $\za_1 = E^a(I_1, B_1)$ be the captured appearance of an input image $I_1$. 
We apply a reconstruction loss between image $I_1$ and cross-cycle reconstruction $\hat{I}_1 = R(B_1, \hat{z}^a_1)$, where $\hat{z}^a_1$ is computed through a cross-cycle with a second image $(I_2, B_2)$, i.e. $\hat{z}^a_1 = E^a(R(B_2, \za_1)), B_2)$.
We also apply a GAN loss on the intermediate appearance transfer output $R(B_2,\za_1)$ as in~\cite{huang2018multimodal,lee2018diverse}.

% Secondly, we add a cross-cycle consistency loss similar to~\cite{lee2018diverse, huang2018multimodal}, where we have a pair of training examples $(B_1, I_1), (B_2, I_2)$ for which we obtain their respective appearance embeddings $\za_1 = E^c(I_1, B_1), \za_2 = E^c(I_2, B_2)$.
% We then apply a 2-step cyclic reconstruction of $I_1, I_2$; In the first step, we rerender both images with a swapped appearance $u = R(B_1, \za_2), v = R(B_2, \za_1)$. In the the second step, we re-capture the latent appearance vectors $\tilde{z}^a_2 = E^a(u, B_1), \tilde{z}^a_1 = E^a(v, B_2)$ and rerender the original images $I_1, I_2$ by swapping the appearance again: $\hat{I}_1 = R(B_1, \tilde{z}^a_1)$, $\hat{I}_2 = R(B_2, \tilde{z}^a_2)$.
% We then use a perceptual loss between the images as the cyclic reconstruction $\mathcal{L}^{\mbox{\scriptsize{vgg}}}(I_i, \hat{I}_i); i \in \{1, 2\}$.

% \begin{itemize}
%     \item 
%     We add a cross-cycle consistency loss~\cite{lee2018diverse, huang2018multimodal}, where we have a pair of training examples $(B_1, I_1), (B_2, I_2)$ for which we obtain their respective appearance embedding $\za_1 = E^c(I_1, B_1), \za_2 = E^c(I_2, B_2)$.
% We then apply a 2-step cyclic reconstruction of $I_1, I_2$; In the first step, we rerender both images with a swapped appearance $u = R(B_1, \za_2), v = R(B_2, \za_1)$. In the the second step, we re-capture the latent appearance vectors $\tilde{\za}_2 = E^a(u, B_1), \tilde{\za}_1 = E^a(v, B_2)$ and rerender the original images $I_1, I_2$ by swapping the appearance again: $\hat{I}_1 = R(B_1, \tilde{\za}_1)$, $\hat{I}_2 = R(B_2, \tilde{\za}_2)$.
% We use a perceptual loss between the images for cyclic reconstruction $\mathcal{L}^{\mbox{\scriptsize{vgg}}}(I_i, \hat{I}_i); i \in \{1, 2\}$.
%$\mathcal{L}^{\mbox{\scriptsize{vgg}}}(I_i, R(B_i, E^a(I_i, B_i))); i \in \{1, 2\}$.
% We apply an LSGAN~\cite{mao2017least} loss between real and rerendered images.
%     \itemize We add an appearance adversarial loss to ensure that the latent appearance vector $\za_i$ doesn't encode any content-related information. ...
% \begin{equation}
%   \begin{split}
% \mathcal{L}^a_{adv} = & \min_{E^a} \max_{D^a} \frac{1}{2} \mathbb{E}_{\za_1, \za_2} \large[ \log(D^a(\za_1 | I^{inp}_1)) + \log(1 - D^a(\za_1 | I^{inp}_2)) \\
% & + \log(D^a(\za_2 | I^{inp}_2)) + \log(1 - D^a(\za_2 | I^{inp}_1))\large]
%   \end{split}
% \end{equation}
% \end{itemize}
% We augment BicycleGAN with the cross-cycle consistency training proposed in~\cite{lee2018diverse, huang2018multimodal}.
% We use the cross-cycle consistency constraint to encourage transferring appearance between two images. This is in contrast to transferring viewpoint
% An alternative to staged training is to jointly train $E^a$ and $R$.

% ------------------------------------------------------------------------------------------------

% \subsubsection{Staged Appearance Training}
% \input{ablative_study}


\paragraph{Staged appearance training}
% We propose a simple yet effective staged approach for multi-modal image translation.
% Our approach avoids joint training of the appearance encoder $E^a$ and rendering network $R$, which is particular challenging as it requires $R$ to discover a correlation between the appearance of an image $I$ and its yet-evolving appearance embedding defined by $E^a$.
% This dynamic can make training unstable, especially at the beginning, as well as more sensitive to hyperparameters.

The key to our staged training approach is the appearance pretraining stage, where we pretrain the appearance encoder $E^a$ independently on a proxy task.
We then train the rendering network $R$ while fixing the weights of $E^a$, allowing $R$ to find the correlations between output images and the embedding produced by the proxy task.
Finally, we fine-tune both $E^a$ and $R$ jointly.


This staged approach simplifies and stabilizes the training of $R$, enabling training of a simpler network with fewer regularization terms.
In particular, we remove the cycle and cross-cycle consistency losses, the latent vector reconstruction loss, and the KL-divergence loss, leaving only a direct reconstruction loss and a GAN loss.
We show experimentally in Section~\ref{sec:evaluation} that this approach results in better appearance capture and rerenderings than the baseline model.

\paragraph{Appearance pretraining}
To pretrain the appearance encoder $E^a$, we choose a proxy task that optimizes an embedding of the input images into the appearance latent space using a suitable distance metric between input images.
This training encourages embeddings such that if two images are close under the distance metric, then their appearance embeddings should also be close in the appearance latent space. 
Ideally the distance metric we choose should ignore the content or viewpoint of $I_i$ and $B_i$, as our goal is to encode a latent space that is independent of viewpoint.
Experimentally we find that the style loss employed in neural style-transfer work~\cite{gatys2016image} has such a property; it largely ignores content and focuses on more abstract properties.

\setlength{\abovedisplayskip}{3pt}
\setlength{\belowdisplayskip}{3pt}

To train the embedding, we use a triplet loss, where for each image $I_i$, we find the set of $k$ closest and furthest neighbor images given by the style loss, from which we can sample a positive sample $I_{p}$ and negative sample $I_{n}$, respectively.
The loss is then:
\[
\mathcal{L}(I_i, I_{p}, I_{n}) = \sum_j \max\left(\|g_i^j\!-\!g_{p}^j\|^2 - \|g_i^j\!-\!g_{n}^j\|^2 + \alpha, 0\right)
\]
where $g^j_i$ is the Gram matrix of activations at the $j^{th}$ layer of a VGG network %\cite{simonyan2014very}
of image $I_i$, and $\alpha$ is a separation margin.





% An alternative to the joint training of the appearance encoder $E^a$ and the rerendering network $R$, we propose a simple, yet effective, staged approach for multi-modal image translation.
% We argue that joint training of $E^a$ and $R$ is challenging.
% During joint training, $E^a$ learns a latent embedding space, while at the same time we require $R$ to discover a correlation between the appearance of an image $I$ and its yet-evolving appearance embedding.
% % A degenerate solution is that $R$ learns to ignore the latent appearance vector $\za$ and associates the appearance of output images with input viewpoints.
% We observe that this makes the training unstable, especially at the beginning, and sensitive to hyperparameters.
% % Alternatively, we propose a simple, yet effective, approach for multimodal image synthesis.
% On the other hand, the staged training comprises three stages:
% (1) Pretraining the appearance encoder, $E^a$, to learn an embedding where images with similar appearance lie closely in that space.
% (2) Fixing $E^a$ while training the rerendering network, $R$.
% And finally (3) finetuning $E^a$ and $R$ together.
% We observe that if a latent embedding space that captures appearance similarity is learned beforehand, then this simplifies and stabilizes the training of the rerendering (generator) network $R$, as it becomes easy for $R$ to learn to associate the target appearance of an image $I$ to its learned latent embedding.
% We pretrain the appearance encoder using a triplet loss. The input is a triplet of images $(I_a, I_{p}, I_{n})$, where $I_a$ is an anchor image, $I_{p}$ has a similar appearance to $I_a$, and $I_{n}$ has a different appearance than $I_a$.
% % $E^a$ then learns an appearance embedding space where images with similar appearance lie close to each other in that embedding space, and lie far from images with different appearance.
% The key to generating triplets is to choose a distance metric between appearances. Then, using this metric we compute the $k$ nearest neighbors and $k$ furthest neighbors for each anchor image $I_a$.
% Triplets are then generated by sampling an anchor image $I_a$ along with one of its $k$-nearest neighbors and one of its $k$-furthest neighbors.
% We experiment with using the style loss employed in neural style transfer~\cite{gatys2016image} as a distance metric. The style loss computes gram matrices for a pair of images using a pretrained VGG~\cite{simonyan2014very} network, and computes the L2 distance between the gram matrices.
% The training loss for $E^a$ is then defined as:
% $$\mathcal{L}^{\mbox{\scriptsize{tri}}}(I_a, I_{\mbox{\scriptsize{p}}}, I_{\mbox{\scriptsize{n}}}) = \sum_{i=1}^N max\huge(\Large[\|g_a^i - g_{\mbox{\scriptsize{p}}}^i\|^2 - \|g_a^i - g_{\mbox{\scriptsize{n}}}^i\|^2 + \alpha \Large], 0\huge)$$ where $g^i$ is the gram matrix computed using the $i^{th}$ layer of the VGG network,  $N$ is the number of layers of the VGG network, and $\alpha$ is a separation margin.
% Visualizing the learned embedding space shows meaningful clustering of different appearances in the training data (see supp.~material).
% After the appearance encoder $E^a$ is trained, we fix its weights and train the rerendering network $R$ in a simple fashion. For an aligned training pair $(B_i, I_i)$, we reconstruct the input image as $\hat{I}_i = R(B_i, E^a(I_i, B_i))$. We then have a LSGAN loss~\cite{mao2017least} between real $I_i$ and fake $\hat{I}_i$ images, as well as a perceptual loss~\cite{johnson2016perceptual} for reconstruction. Our results show that the proposed staged training learns a better appearance model than our baseline as we discuss in Section~\ref{sec:?}.


% it better captures the appearance and shows complex appearance interpolation.
% On the other hand, the baseline learns a simple appearance model, where interpolating between two appearances resembles a linear interpolation of between two aligned images in the pixel domain.
% Note that this is not very powerful, as this doesn't capture complex appearance transitions like shadows, lights, ..


% =================================================================================================



\subsection{Semantic conditioning}
\label{sec:semantic_conditioning}

To account for transient objects in the scene, we condition the rerendering network on a semantic labeling $S_i$ of image $I_i$ that depicts the location of transient objects such as pedestrians.
% To condition the network,
Specifically,
we concatenate the semantic labeling $S_i$ to the deep buffer $B_i$ wherever the deep buffer was previously used.
This discourages the network from encoding variations caused by the location of transient objects in the appearance vector, or associating such transient objects with specific viewpoints, as shown in Figure~\ref{fig:pix2pix_limitations}.

A separate benefit of semantic labeling is that it allows the rerendering network to reason about static objects in the scene not captured in the 3D reconstruction, such as lampposts in San Marco Square.
% Rather than introducing such objects haphazardly, the network is guided by the semantic labels
This prevents the network from haphazardly introducing such objects, and instead lets them appear where they are detected in the semantic labeling, which is a significantly simpler task.
In addition, by adding the segmentation labeling to the deep buffer, we allow the appearance encoder to reason about semantic categories like sky or ground when computing the appearance latent vector. 

We compute ``ground truth'' semantic segmentations on the input images $I_i$ using DeepLab~\cite{chen2018deeplab} trained on ADE20K~\cite{zhou2017scene}.
ADE20K contains 150 classes, which we map to a 3-channel color image.
We find that the quality of the semantic labeling is poor on the landmarks themselves, as they contain unique buildings and features, but is reasonable on transient objects.

Using semantic conditioning, the rerendering network takes as input a semantic labeling of the scene.
In order to rerender virtual camera paths, we need to synthesize semantic labelings for each frame in the virtual camera path.
To do so, we train a separate semantic labeling network that takes as input the deep buffer $B_i$, instead of the output image $I_i$, and estimates a ``plausible'' semantic labeling $\hat{S}_i$ for that viewpoint given the rendered deep buffer $B_i$. 
For simplicity, we train a network with the same architecture as the rendering network (minus the injected appearance vector) on samples $(B_i,S_i)$ from the aligned dataset, and we modify the semantic labelings of the ground truth images $S_i$ and mask out the loss on pixels labeled as transient as defined by a curated list of transient object categories in ADE20K.


% During training, a real image could contain several transient objects that are not part of the corresponding rendered viewpoint.
% So, the network learns to encode variations caused by transient objects in the appearance vector $\za$, or worse, it can associate such transient objects with the input viewpoint $B_i$.
% At test time, and for an unseen viewpoint, the network then hallucinates transient objects and their positions.
% This is shown in Figure~\ref{fig:baseline} where a simple pix2pix network hallucinates multiple lampposts (left image) or people (middle and right images).
% %
% So, we aim to eliminate the guessing of the network by augmenting the input deep buffer $B_i$ with an extra semantic segmentation map $S_i$ that specifies which semantic objects the network should render and where to render them.
% %
% At training time, we segment training images using an off-the-shelf semantic segmentation model.
% %
% Specifically, we use a semantic segmentation network trained on the ADE20K dataset~\cite{zhou2017scene} using Deeplab~\cite{chen2018deeplab}.
% ADE20K contains a mix indoor and urban outdoor scenes, which are quite different compared to the tourist landmarks we evaluate our system. 
% This makes the quality of the segmentations on our dataset quite poor.
% However, we note that with large enough training data, our rerendering network eventually learns to reason correctly about the input segmentation map.
% %
% % A byproduct to having a segmentation map as an input is that we can perform semantic manipulations on the output image by modifying the input segmentation as shown in Section~\ref{sec:exp_semantics}.
% % =================================================================================================
% At test time, we need to generate semantic segmentation masks for novel viewpoints, for which we don't have a corresponding ground truth image to segment. So, we train an image translation network $S(B_i)$ that takes as input the deep buffer $B_i$ and outputs a \emph{plausible} segmentation mask $S_i$ for that viewpoint.
% To prevent this network from hallucinating the location of transient objects in the scene, we mask such pixels in the input and output segmentation masks and train the network with an L1 reconstruction loss.
% This is sufficiently effective to produce good segmentation masks for synthesizing virtual camera paths of the scene. A byproduct to conditioning the rerendering on the the segmentation mask is that we can perform simple semantic manipulation, such as removing objects or moving them around, by moeifying the input segmentation mask



==> tables/generalized_pretraining.tex <==
\begin{table*}[t!]
\centering
\begin{footnotesize}
\caption{Generalization of a pretrained style encoder $E$. We report validation set reconstruction for the edges2handbags and night2day datasets when pretraining with different datasets. Stages 2, 3 show results before/after finetuning $E$ respectively.}
\label{table:generalize_enc}
% \vspace{-0.1in}
\resizebox{0.55\linewidth}{!}{
    \begin{tabular}{@{}llcccc@{}}
    \toprule % \hline
    % Dataset & pretrain dataset & L1 & LPIPS \\ \hline
    \multirow{2}{*}{Dataset} & \multirow{2}{*}{pretrain dataset} & \multicolumn{2}{c}{Stage 2} & \multicolumn{2}{c}{Stage 3} \\ \cmidrule{3-6}
    & & PSNR $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & LPIPS $\downarrow$ \\ \midrule
    \multirow{3}{*}{edges2handbags} & edges2handbags & 18.01 & 0.209 & 18.91 & 0.177 \\ %\cline{2-6}
    & edges2shoes & 17.89 & 0.215 & 18.96 & 0.176 \\ %\cline{2-6}
    & space\_needle  & 17.86 & 0.221 & 19.02 & 0.175 \\ \midrule %\hline
    \multirow{3}{*}{night2day} & night2day & 13.75 & 0.489 & 15.15 & 0.454 \\ %\cline{2-6}
    & space\_needle & 14.34 & 0.476 & 15.05 & 0.452 \\ %\cline{2-6}
    & edges2handbags & 13.91 & 0.492 & 15.03 & 0.461 \\ \bottomrule
    \end{tabular}
}
% \vspace{-0.2in}
% \vspace{-0.12in}
\end{footnotesize}
\end{table*}


% ------------------------------------------------------------------------------

% \begin{table*}[t!]
% \centering
% \begin{footnotesize}
% \caption{Generalization of a pretrained style encoder $E$. We report validation set reconstruction and Inception Score (IS) for the edges2handbags and night2day datasets when pretraining with different datasets. Stages 2, 3 show results before/after finetuning $E$ respectively.}
% \label{table:generalize_enc}
% \vspace{-0.1in}
% \resizebox{0.8\linewidth}{!}{
%     \begin{tabular}{@{}llcccccc@{}}
%     \toprule % \hline
%     % Dataset & pretrain dataset & L1 & LPIPS \\ \hline
%     \multirow{2}{*}{Dataset} & \multirow{2}{*}{pretrain dataset} & \multicolumn{2}{c}{Stage 2} & \multicolumn{2}{c}{Stage 3} \\ \cmidrule{3-8}
%                               &                & PSNR $\uparrow$ & IS $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & IS $\uparrow$ & LPIPS $\downarrow$ \\ \midrule
%     \multirow{3}{*}{handbags}  & handbags       & 18.01           & 2.52          & 0.209         & 18.91                & 2.39          & 0.177 \\ %\cline{2-6}
%                               & shoes          & 17.89           & 2.44          & 0.215         & 18.96                & 2.42          & 0.176 \\ %\cline{2-6}
%                               & space\_needle  & 17.86           & 2.60          & 0.221         & 19.02                & 2.48          & 0.175 \\ \midrule %\hline
%     \multirow{3}{*}{night2day} & night2day      & 13.75           & 2.61          & 0.489         & 15.15                & 2.77          & 0.454 \\ %\cline{2-6}
%                               & space\_needle  & 14.34           & 2.55          & 0.476         & 15.05                & 2.45          & 0.452 \\ %\cline{2-6}
%                               & handbags       & 13.91           & 2.53          & 0.492         & 15.03                & 2.43          & 0.461 \\ \bottomrule
%     \end{tabular}
% }
% \vspace{-0.25in}
% \end{footnotesize}
% \end{table*}

